Carbon-aware Software Services

The significant carbon footprint of the ICT sector calls for methodologies to contain carbon emissions of running software. This article proposes a novel framework for implementing, configuring and assessing carbon-aware interactive software services. First, we propose a methodology to implement carbon-aware services leveraging the Strategy design pattern to feature alternative service versions with different energy consumption. Then, we devise a bilevel optimisation scheme to configure which version to use at different times of the day, based on forecasts of carbon intensity and service requests, pursuing the two-fold goal of minimising carbon emissions and maintaining average output quality above a desired set-point. Last, an open-source prototype of such optimisation scheme is used to configure a software service implemented as per our methodology and assessed against traditional non-adaptive implementations of the same service. Results show the capability of our framework to control the average quality of output results of carbon-aware services and to reduce carbon emissions from 8% to 50%.

==> macro.tex <==
%% The amssymb package provides various useful mathematical symbols
\usepackage{amssymb}
\usepackage[dvipsnames]{xcolor}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{xcolor}
\usepackage{tabularx}
\usepackage{verbatim}
\usepackage{xspace}
\usepackage{fancyvrb}
\usepackage{fvextra}
\usepackage{subcaption}
\usepackage{inconsolata}
\usepackage{colortbl}
\usepackage{url}
\usepackage{hyperref}
\usepackage{wrapfig}
\usepackage{placeins}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{float}
\usepackage{breqn}
\usepackage{csquotes}

\usepackage{tikz}
\usepackage{tkz-graph}
\usepackage{eurosym}
\usetikzlibrary{calc,shapes.multipart,chains,arrows}
\usetikzlibrary{arrows,automata}
\usetikzlibrary{positioning}




\usepackage[normalem]{ulem}
\newcommand{\togliere}[1]{\textcolor{orange}{\sout{#1}}}

%% The amsthm package provides extended theorem environments
%\usepackage{mathtools}%add-on and patches to amsmath
\usepackage{amsthm}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{example}{Example}
\usepackage{cleveref}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}

% Bibliography 
\usepackage[english]{babel}

% :- 
\newcommand{\impl}{\ {:\!-}\  }
% :~
\newcommand{\wc}{\ {:\sim}\  }

\everymath{\displaystyle}

\renewcommand\UrlFont{\color{blue}\rmfamily}

% cleveref re-label
\crefname{section}{Section}{Section}
\Crefname{section}{Section}{Section}
\crefname{figure}{Figure}{Figure}
\Crefname{figure}{Figure}{Figure}
\crefname{table}{Table}{Table}
\Crefname{table}{Table}{Table}

\let\cleardoublepage\clearpage
\newcommand{\pptext}[1]{\smallskip\noindent \textit{#1}\xspace} 
\newcommand{\cd}[1]{\texttt{\small #1}\xspace}
%\newcommand{\cd}[1]{$\mathit{#1}$\xspace}
\newcommand{\fncd}[1]{\texttt{\footnotesize #1}\xspace} % code in footnotes
\newcommand{\diam}{\hfill$\diamond$}
\newcommand{\proimg}{\xspace{\sf declace}\xspace}
\newcommand{\plnot}{{\scriptsize\textbackslash}+}
\newcommand{\clingo}{\textsc{clingo}\xspace}
\newcommand{\atterm}{\textit{@}-term\xspace}
\newcommand{\atterms}{\textit{@}-terms\xspace}


% verbatim environment for prolog code
\DefineVerbatimEnvironment{code}{Verbatim}
{fontfamily=zi4, fontsize=\footnotesize, frame=single, framesep=1mm, framerule=0.1pt, rulecolor=\color{gray}}

\DefineVerbatimEnvironment{codeNum}{Verbatim}

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

 % \newcommand{\textapprox}{\raisebox{0.5ex}{\texttildelow}}


% plot
\usepackage{tkz-graph}
\usepackage{pgfplots}
\usepackage{subcaption} 
\usepackage{tkz-graph}

\usepackage{multirow}

\usepackage{xcolor}
\newcommand{\red}[1]{\textcolor{red}{#1}}

% \definecolor{red_plot}{HTML}{F30522}
\definecolor{first_color_plot}{HTML}{F30522}

% \definecolor{green_plot}{HTML}{20D525}
\definecolor{second_color_plot}{HTML}{20D525}

% \definecolor{yellow_plot}{HTML}{DED712}
\definecolor{third_color_plot}{HTML}{DED712}

% \definecolor{blue_plot}{HTML}{67A9CF}
\definecolor{fourth_color_plot}{HTML}{67A9CF}

\definecolor{orange_plot}{HTML}{FA5F22}
\definecolor{pink_plot}{HTML}{FFD0B4}
\definecolor{light_blue_plot}{HTML}{D1E5F0}
\definecolor{dark_blue_plot}{HTML}{2166AC}

\newcommand{\textwidthresizebox}{0.40}
\newcommand{\alignedimgsresizebox}{0.85}

\usepackage{tikz}
\usetikzlibrary{shapes.geometric, arrows}

\tikzstyle{start} = [circle,draw=black]

% \tikzstyle{io} = [trapezium, 
% % trapezium stretches=true, % A later addition
% trapezium left angle=70, 
% trapezium right angle=110, 
% minimum width=3cm, 
% minimum height=1cm, text centered, 
% draw=black]

\tikzstyle{process} = [rectangle, 
minimum width=3cm, 
minimum height=1cm, 
text centered, 
text width=3cm, 
draw=black]

\tikzstyle{wf_node} = [rectangle, 
minimum width=1cm, 
minimum height=1cm, 
text centered, 
text width=2cm, 
draw=black,
rounded corners]


\tikzstyle{decision} = [diamond, 
minimum width=3cm, 
minimum height=1cm, 
text centered, 
text width=2cm, 
draw=black]
\tikzstyle{arrow} = [thick,->,>=stealth]

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}
